Low-Latency Sequence-to-Sequence Speech Recognition and Translation by Partial Hypothesis Selection

Encoder-decoder models provide a generic architecture for sequence-to-sequence tasks such as speech recognition and translation. While offline systems are often evaluated on quality metrics like word error rates (WER) and BLEU, latency is also a crucial factor in many practical use-cases. We propose three latency reduction techniques for chunk-based incremental inference and evaluate their efficiency in terms of accuracy-latency trade-off. On the 300-hour How2 dataset, we reduce latency by 83% to 0.8 second by sacrificing 1% WER (6% rel.) compared to offline transcription. Although our experiments use the Transformer, the hypothesis selection strategies are applicable to other encoder-decoder models. To avoid expensive re-computation, we use a unidirectionally-attending encoder. After an adaptation procedure to partial sequences, the unidirectional model performs on-par with the original model. We further show that our approach is also applicable to low-latency speech translation. On How2 English-Portuguese speech translation, we reduce latency to 0.7 second (-84% rel.) while incurring a loss of 2.4 BLEU points (5% rel.) compared to the offline system.

==> sections/acknolwedge.tex <==
Authors should not use logos in acknowledgement section; rather authors should acknowledge corporations by naming them only.

==> tabs/beforeAdapt.tex <==
\begin{table*}
	\footnotesize
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{@{}>{\raggedleft\arraybackslash}p{1.9cm}rrrrrrrrrrr@{}}
			\toprule
			& 
			\multicolumn{5}{c}{\textbf{Baseline}} && \multicolumn{5}{c}{\textbf{Unidirectional}} \\
			\cmidrule{2-6} \cmidrule{8-12}
			\multirow{2}{*}{\textbf{\makecell[bl]{Dataset, \\ Strategies}}} & \multicolumn{2}{c}{dev} && \multicolumn{2}{c}{test} && \multicolumn{2}{c}{dev} && \multicolumn{2}{c}{test} \\
			\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
			& \makecell[c]{WER \\ (\%)} & \makecell[c]{$\Delta$ latency \\ (seconds)} && \makecell[c]{WER \\ (\%)} & \makecell[c]{$\Delta$ latency \\ (seconds)} && \makecell[c]{WER \\ (\%)} & \makecell[c]{$\Delta$ latency \\ (seconds)} && \makecell[c]{WER \\ (\%)} & \makecell[c]{$\Delta$ latency \\ (seconds)} \\
			\midrule
			hold 0 & 37.7  &  0    && \textbf{37.4}  &  0    && 41.3 &  0    && 40.7 &  0    \\	
			\midrule
			\multicolumn{1}{l}{\textbf{Hold-$n$}} &&&&&&&&&&& \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{28.3}  & +0.32 &&      &       && 30.3 & +0.30 \\
			hold 2 & 22.0  & +0.33 && \textbf{20.4}  & +0.48 && 25.3 & +0.15 && 22.0 & +0.42 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{18.7}  & +0.77 &&      &       && 19.3 & +0.74 \\
			hold 4 & 18.8  & +0.74 && \textbf{17.8}  & +0.92 && 21.7 & +0.57 && 18.8 & +0.83 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{17.1}  & +1.22 &&      &       && 17.3 & +1.16 \\
			hold 6 & 18.1  & +1.14 && \textbf{16.8}  & +1.34 && 20.6 & +0.93 && 17.6 & +1.22 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{16.5}  & +1.60 &&      &       && \textbf{16.5} & +1.52 \\
			hold 8 & 17.8 & +1.49  && \textbf{16.4}  & +1.71 && 19.8 & +1.25 && 17.2 & +1.58 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && 16.2           & +1.96 &&      &       && \textbf{16.1} & +1.88 \\
			hold 10 & 17.6 & +1.81 && \textbf{16.2}  & +2.04 && 19.7 & +1.56 && 16.8 & +1.92 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && 16.1           & +2.27 &&      &       && \textbf{15.8} & +2.19 \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multicolumn{1}{l}{\textbf{Wait-$k$}} &&&&&&&&&&& \\
			rate 2         & 16.7 & +2.19 && \textbf{17.0} & +2.24 && 16.8 & +2.18 && \textbf{16.8} & +2.24 \\	
			rate 4         & 20.2 & +0.74 && \textbf{20.3} & +0.72 && 20.3 & +0.66 && 20.7 & +1.06 \\
			rate 6         & 26.5 & +0.34 && 26.7 & +0.30 && 27.7 & +0.23 && \textbf{26.1} & +0.81 \\
			rate 8         & 31.2 & +0.22 && 31.3 & +0.18 && 33.1 & +0.11 && \textbf{29.7} & +0.71 \\
			rate 2 + $k$   & 15.5 & +2.37 && 15.9 & +2.44 && 17.0 & +2.49 && \textbf{15.4} & +2.37 \\
			rate 4 + $k$   & 17.6 & +0.95 && \textbf{18.0} & +0.94 && 19.3 & +1.08 && 18.5 & +1.04 \\
			rate 6 + $k$   & 23.0 & +0.50 && 23.2 & +0.48 && 25.8 & +0.64 && \textbf{22.9} & +0.71 \\
			rate 8 + $k$   & 27.3 & +0.36 && 27.3 & +0.34 && 30.7 & +0.50 && \textbf{25.7} & +0.68 \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multicolumn{1}{l}{\textbf{Output-if-agree}} &&&&&&&&&&& \\	
			- & 15.5 & +0.79 && \textbf{15.8} & +0.81 && 19.7 & +0.44 && 16.8 & +0.54 \\	
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\midrule
			\textcolor{oCl}{offline} & \textcolor{oCl}{14.4} & \textcolor{oCl}{+4.40} && \textcolor{oCl}{14.9} & \textcolor{oCl}{+4.55} && \textcolor{oCl}{14.2} &     \textcolor{oCl}{+4.31} && \textcolor{oCl}{14.4} & \textcolor{oCl}{+4.47} \\
			\bottomrule
		\end{tabular}
	}
	\caption{Online decoding performance of the wait-$k$ strategy, with varying output rates (tokens per second). ``$+k$'' indicates waiting for the first 0.5-second chunk. The hold-$0$ strategy provides the upper bound for word error rate and lower bound for latency. The two ``$+0.00$'' entries are due to rounding down.}
	\label{tab.waitK}
\end{table*}

==> tabs/beforeAfterAdapt.tex <==
\begin{table*}
	\caption{Online decoding performance of the wait-$k$ strategy, with varying output rates (tokens per second). ``$+k$'' indicates waiting for the first 0.5-second chunk. The hold-$0$ strategy provides the upper bound for word error rate and lower bound for latency.}
	\footnotesize
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{@{}>{\raggedleft\arraybackslash}p{1.8cm}rrrrrrrrrrrrrrrrrr@{}}
			\toprule
			\multirow{2}{*}{\makecell[bl]{Strategies, \\ hyperparameters}} &  
			\multicolumn{5}{c}{\textbf{Bidirectional}} && \multicolumn{5}{c}{\textbf{Unidirectional}} \\
			\cmidrule{2-6} 
			\cmidrule{8-12}
			&
			\multicolumn{2}{c}{Before Adaptation} && 
			\multicolumn{2}{c}{After Adaptation} &&
			\multicolumn{2}{c}{Before Adaptation} && 
			\multicolumn{2}{c}{After Adaptation} \\
			\cmidrule{2-3} 
			\cmidrule{5-6} 
			\cmidrule{8-9} 
			\cmidrule{11-12}
			& 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} \\
			\midrule
			Hold-0 & 37.7, \textbf{37.4}  &  0, 0    && ...  &  ...  && 41.3, 40.7 &  0, 0 && ... & ... \\
%			\multicolumn{1}{l}{\textbf{Hold-$n$}} &&&&&&&&&&& \\
		 	Hold-2 & 22.0, \textbf{20.4} & +0.33, +0.48 && ... & ... && 25.3, 22.0 & +0.15, +0.42 && ... & ... \\
			Hold-4 & 18.8, \textbf{17.8} & +0.74, +0.92 && ... & ... && 21.7, 18.8 & +0.57, +0.83 &&  &  \\
%			hold 6 & 18.1, \textbf{16.8} & +1.14, +1.34 && ... & ... && 20.6, 17.6 & +0.93, +1.22 &&  &  \\
%			hold 8 & 17.8, \textbf{16.4} & +1.49, +1.71  && ... & ... && 19.8, 17.2 & +1.25, +1.58 && ... &  \\
%			hold 10 & 17.6, \textbf{16.2} & +1.81, +2.04 && ... & ... && 19.7, 16.8 & +1.56, +1.92 && ... & ... \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%			\multicolumn{1}{l}{\textbf{Output-if-agree}} &&&&&&&&&&& \\	
			Hyp. stability & 15.5, \textbf{15.8} & +0.79, +0.81 && ... & ... && 19.7, 16.8 & +0.44, +0.54 && ... &  \\	
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%			\multicolumn{1}{l}{\textbf{Wait 1 chunk}} &&&&&&&&&&& \\
%			rate 2         & 16.7 & +2.19 && \textbf{17.0} & +2.24 && 16.8 & +2.18 && \textbf{16.8} & +2.24 \\	
%			rate 4         & 20.2 & +0.74 && \textbf{20.3} & +0.72 && 20.3 & +0.66 && 20.7 & +1.06 \\
%			rate 6         & 26.5 & +0.34 && 26.7 & +0.30 && 27.7 & +0.23 && \textbf{26.1} & +0.81 \\
%			rate 8         & 31.2 & +0.22 && 31.3 & +0.18 && 33.1 & +0.11 && \textbf{29.7} & +0.71 \\
%			rate 2   & 15.5, 15.9 & +2.37, +2.44 && ... & ... && 17.0, \textbf{15.4} & +2.49, +2.37 && ... & ... \\
%			rate 4   & 17.6, \textbf{18.0} & +0.95, +0.94 && ... & ... && 19.3, 18.5 & +1.08, +1.04 &&  ... & ... \\
%			rate 6   & 23.0, 23.2 & +0.50, +0.48 && ... & ... && 25.8, \textbf{22.9} & +0.64, +0.71 && ... & ... \\
%			rate 8   & 27.3, 27.3 & +0.36, +0.34 && ... & ... && 30.7, \textbf{25.7} & +0.50, +0.68 &&  ... & ... \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			Offline & 14.4, 14.9 & +4.40, +4.55 && ... & ... && 14.2, 14.4 &     +4.31, +4.47 && \textcolor{oCl}{...} & \textcolor{oCl}{...} \\
			\bottomrule
		\end{tabular}
	}
	\label{tab.full}
\end{table*}

==> tabs/beforeAfterAdapt__copy_.tex <==
\begin{table*}
	\footnotesize
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{@{}>{\raggedleft\arraybackslash}p{2.2cm}rrrrrrrrrrrrrrrrrr@{}}
			\toprule
			& 
			\multicolumn{5}{c}{\textbf{Bidirectional}} && \multicolumn{5}{c}{\textbf{Unidirectional}} \\
			\cmidrule{2-6} 
			\cmidrule{8-12}
			\multirow{2}{*}{\makecell[bl]{Decoding strategies, \\ hyperparameters}} & 
			\multicolumn{2}{c}{dev} && 
			\multicolumn{2}{c}{test} &&
			\multicolumn{2}{c}{dev} && 
			\multicolumn{2}{c}{test} \\
			\cmidrule{2-3} 
			\cmidrule{5-6} 
			\cmidrule{8-9} 
			\cmidrule{11-12}
			& 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} && 
			\makecell[c]{WER (\%)} & \makecell[c]{$\Delta$ latency (sec.)} \\
			\midrule
			hold 0 & 37.7  &  0    && \textbf{37.4}  &  0    && 41.3 &  0    && 40.7 &  0    \\	
			\midrule
			\multicolumn{1}{l}{\textbf{Hold-$n$}} &&&&&&&&&&& \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{28.3}  & +0.32 &&      &       && 30.3 & +0.30 \\
			hold 2 & 22.0  & +0.33 && \textbf{20.4}  & +0.48 && 25.3 & +0.15 && 22.0 & +0.42 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{18.7}  & +0.77 &&      &       && 19.3 & +0.74 \\
			hold 4 & 18.8  & +0.74 && \textbf{17.8}  & +0.92 && 21.7 & +0.57 && 18.8 & +0.83 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{17.1}  & +1.22 &&      &       && 17.3 & +1.16 \\
			hold 6 & 18.1  & +1.14 && \textbf{16.8}  & +1.34 && 20.6 & +0.93 && 17.6 & +1.22 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && \textbf{16.5}  & +1.60 &&      &       && \textbf{16.5} & +1.52 \\
			hold 8 & 17.8 & +1.49  && \textbf{16.4}  & +1.71 && 19.8 & +1.25 && 17.2 & +1.58 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && 16.2           & +1.96 &&      &       && \textbf{16.1} & +1.88 \\
			hold 10 & 17.6 & +1.81 && \textbf{16.2}  & +2.04 && 19.7 & +1.56 && 16.8 & +1.92 \\
			%		 \rowcolor{Gray}
			%		 + adapt&       &       && 16.1           & +2.27 &&      &       && \textbf{15.8} & +2.19 \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multicolumn{1}{l}{\textbf{Wait-$k$}} &&&&&&&&&&& \\
			rate 2         & 16.7 & +2.19 && \textbf{17.0} & +2.24 && 16.8 & +2.18 && \textbf{16.8} & +2.24 \\	
			rate 4         & 20.2 & +0.74 && \textbf{20.3} & +0.72 && 20.3 & +0.66 && 20.7 & +1.06 \\
			rate 6         & 26.5 & +0.34 && 26.7 & +0.30 && 27.7 & +0.23 && \textbf{26.1} & +0.81 \\
			rate 8         & 31.2 & +0.22 && 31.3 & +0.18 && 33.1 & +0.11 && \textbf{29.7} & +0.71 \\
			wait 1 chunk, rate 2   & 15.5 & +2.37 && 15.9 & +2.44 && 17.0 & +2.49 && \textbf{15.4} & +2.37 \\
			wait 1 chunk, rate 4   & 17.6 & +0.95 && \textbf{18.0} & +0.94 && 19.3 & +1.08 && 18.5 & +1.04 \\
			wait 1 chunk, rate 6   & 23.0 & +0.50 && 23.2 & +0.48 && 25.8 & +0.64 && \textbf{22.9} & +0.71 \\
			wait 1 chunk, rate 8   & 27.3 & +0.36 && 27.3 & +0.34 && 30.7 & +0.50 && \textbf{25.7} & +0.68 \\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multicolumn{1}{l}{\textbf{Output-if-agree}} &&&&&&&&&&& \\	
			- & 15.5 & +0.79 && \textbf{15.8} & +0.81 && 19.7 & +0.44 && 16.8 & +0.54 \\	
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\midrule
			\textcolor{oCl}{offline} & \textcolor{oCl}{14.4} & \textcolor{oCl}{+4.40} && \textcolor{oCl}{14.9} & \textcolor{oCl}{+4.55} && \textcolor{oCl}{14.2} &     \textcolor{oCl}{+4.31} && \textcolor{oCl}{14.4} & \textcolor{oCl}{+4.47} \\
			\bottomrule
		\end{tabular}
	}
	\caption{Online decoding performance of the wait-$k$ strategy, with varying output rates (tokens per second). ``$+k$'' indicates waiting for the first 0.5-second chunk. The hold-$0$ strategy provides the upper bound for word error rate and lower bound for latency. The two ``$+0.00$'' entries are due to rounding down.}
	\label{tab.waitK}
\end{table*}

==> tabs/offline.tex <==
\begin{table}[h]
	\footnotesize
	\centering
	\caption{Offline inference word and error rates (\%) of the baseline and unidirectional.}
	\begin{tabular}{@{}lcccccccccccc@{}}
		\toprule
		\multirow{2}{*}{Strategies} & \multicolumn{2}{c}{\textbf{Baseline}} && \multicolumn{2}{c}{\textbf{Unidirectional}} && \multicolumn{2}{c}{\textbf{Baseline}} && \multicolumn{2}{c}{\textbf{Unidirectional}}\\
		\cmidrule{2-3} \cmidrule{5-6} 
		& \multicolumn{1}{c}{WER} & \multicolumn{1}{c}{latency} && \multicolumn{1}{c}{WER} & \multicolumn{1}{c}{latency} \\
		%		\cmidrule{2-5} \cmidrule{7-10}
		%		& WER & CER & WER & CER && WER & CER & WER & CER \\
		\midrule
		hold-0  & 37.4  &  0    &&  &  \\
		hold-4  & 17.8  & +0.9  && 18.8 & +0.8 \\
		if-agree& 15.8  & +0.8  && 16.8 & +0.5 \\ 
		offline & 14.9  & +4.6  && 14.4 & +4.5 \\
		%		Libri & 7.0 & 3.6 & \textbf{9.2}  & \textbf{4.7} && 7.9  & 3.4 & 9.7  & 4.3\\
		\bottomrule
	\end{tabular}
	\label{tab.bounds}
\end{table}
